DEEPCHART: How Far are LLMs from Faithful Data-Science Chart Generation?

Faithful chart generation in real-world data-science workflows requires grounding visualizations in scattered evidence, computing chart-ready quantities, and rendering them accurately. Modern LLMs can produce visually plausible, instruction-compliant charts, yet data-level hallucinations remain difficult to detect in long, noisy, and multimodal contexts. To measure this gap, we introduce DEEPCHART, an expert-annotated benchmark of 1,482 task-conditioned chart-generation instances drawn from real-world scientific papers, financial filings, and ecosystem reports. DEEPCHART formulates chart generation as an Extract--Reason--Visualize pipeline and evaluates source-data extraction, derived-data reasoning, and chart rendering stage by stage. Experiments with state-of-the-art models show that visually plausible charts often conceal data-level hallucinations, with extraction and reasoning errors common in realistic long and multimodal settings. These findings suggest that larger context windows alone are insufficient; faithful chart generation also requires reliable evidence extraction and quantitative reasoning before rendering. Our benchmark and associated resources are available at https://github.com/tangdouer1005/DeepChart.

==> latex/table/bench_token.tex <==
\begin{table}[t]
\centering
\small
% 增加行高，让表格看起来更舒展
\renewcommand{\arraystretch}{1.15}
% 适当调整列间距
\setlength{\tabcolsep}{4pt}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{llrrr}
\toprule
\multirow{2}{*}{\textbf{Domain} ($N$)} & \multirow{2}{*}{\textbf{Level}} & \multicolumn{3}{c}{\textbf{Context Length (Tokens)}} \\
\cmidrule(lr){3-5}
 & & \textbf{Mean} & \textbf{Min} & \textbf{Max} \\
\midrule
\multirow{3}{*}{Academic (178)} 
 & Short & 5,872 & 111 & 67,199 \\
 & Medium & 80,766 & 14,788 & 166,579 \\
 & Long $^\dagger$ & -- & -- & -- \\
\midrule
\multirow{3}{*}{Finance (284)} 
 & Short & 34,992 & 19,146 & 47,961 \\
 & Medium & 137,729 & 68,354 & 197,337 \\
 & \textbf{Long} & \textbf{700,858} & \textbf{242,472} & \textbf{1,196,230} \\
\bottomrule
\end{tabular}}
\caption{Statistics of input context length. The \textbf{Long} setting in the Finance domain involves full 10-K reports. $^\dagger$Note: Academic papers typically do not reach the threshold for the "Long" setting.}
\vspace{-1.\baselineskip}
\label{tab:token_stats}
\end{table}

==> latex/table/e3.tex <==



\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{3pt} % 紧凑列宽
    \renewcommand{\arraystretch}{1.1}
    
    \begin{tabular}{ll cccc}
        \toprule
        \textbf{Model} & \textbf{Paradigm} & \textbf{$F_{1,\mathrm{src}}$} & \textbf{$F_{1,\mathrm{der}}$} & \textbf{VAS} & \textbf{ER} \\
        \midrule
        
        % --- GPT-5.2 ---
        \multirow{2}{*}{\textbf{GPT-5.2}} 
         & One-Step & \multicolumn{2}{c}{\textit{\textcolor{gray}{N/A (Black Box)}}} & 88.5 & \textbf{98.9} \\
         & \textbf{Two-Step} & \textbf{92.5} & \textbf{89.4} & \textbf{94.1} & 98.5 \\
        \cmidrule(lr){1-6}
        
        % --- DeepSeek ---
        \multirow{2}{*}{\textbf{DeepSeek}} 
         & One-Step & \multicolumn{2}{c}{\textit{\textcolor{gray}{N/A (Black Box)}}} & 84.2 & \textbf{97.5} \\
         & \textbf{Two-Step} & \textbf{88.9} & \textbf{85.8} & \textbf{90.5} & 96.8 \\
        \cmidrule(lr){1-6}
        
        % --- Qwen ---
        \multirow{2}{*}{\textbf{Qwen3}} 
         & One-Step & \multicolumn{2}{c}{\textit{\textcolor{gray}{N/A (Black Box)}}} & 81.0 & \textbf{96.5} \\
         & \textbf{Two-Step} & \textbf{89.5} & \textbf{86.2} & \textbf{87.2} & 95.8 \\
        
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Ablation on Generation Paradigms.} 
        Results are \textbf{averaged} across Finance and Academic domains.
        The \textbf{One-Step} baseline lacks intermediate data, making F1 metrics inapplicable (N/A) and rendering the reasoning process opaque.
        Our \textbf{Two-Step} paradigm unlocks diagnosability (F1 scores) and significantly boosts visual logic (VAS) across all models.
    }
    \label{tab:ablation-paradigm}
\end{table}

==> latex/table/shared_setting.tex <==
\begin{table*}[t]
    \renewcommand\arraystretch{1.15}
    \small
    \centering
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{3}{c|}{\textbf{Finance Domain Avg.}}
        & \multicolumn{3}{c|}{\textbf{Academic Domain Avg.}}
        & \multicolumn{3}{c}{\textbf{Ecosystem Domain}} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}

        & \textbf{$F_{1,\mathrm{src}}$} & \textbf{$F_{1,\mathrm{der}}$} & \textbf{VAS}
        & \textbf{$F_{1,\mathrm{src}}$} & \textbf{$F_{1,\mathrm{der}}$} & \textbf{VAS}
        & \textbf{$F_{1,\mathrm{src}}$} & \textbf{$F_{1,\mathrm{der}}$} & \textbf{VAS} \\
        \midrule

        GPT-5.2
        & 0.3357 & 0.2705 & 0.4812
        & 0.6623 & 0.1885 & 0.5093
        & 0.0207 & 0.0386 & 0.1589 \\

        Claude 4.5 Opus
        & 0.3286 & 0.1758 & 0.4947
        & 0.7009 & 0.2071 & \textbf{0.5974}
        & 0.1792 & 0.2832 & 0.6963 \\

        Gemini 3 Pro
        & \textbf{0.4664} & 0.3418 & 0.3889
        & \textbf{0.7207} & 0.2416 & 0.2940
        & 0.1965 & \textbf{0.4529} & \textbf{0.7427} \\

        Gemini 3 Flash
        & 0.4621 & \textbf{0.4597} & \textbf{0.5155}
        & 0.7054 & \textbf{0.2480} & 0.4052
        & \textbf{0.2167} & 0.4107 & 0.4055 \\

        \bottomrule
    \end{tabular}
    }
\caption{\textbf{Cross-domain comparison on shared models.} Finance and Academic scores are macro-averaged over their available context settings; Ecosystem scores are reported under the native multimodal setting.}

\label{tab:shared_setting}
\end{table*}

